Diversity-aware clustering: Computational Complexity and Approximation Algorithms

In this work, we study diversity-aware clustering problems where the data points are associated with multiple attributes resulting in intersecting groups. A clustering solution needs to ensure that the number of chosen cluster centers from each group should be within the range defined by a lower and upper bound threshold for each group, while simultaneously minimizing the clustering objective, which can be either $k$-median, $k$-means or $k$-supplier. We study the computational complexity of the proposed problems, offering insights into their NP-hardness, polynomial-time inapproximability, and fixed-parameter intractability. We present parameterized approximation algorithms with approximation ratios $1+ \frac{2}{e} + \epsilon \approx 1.736$, $1+\frac{8}{e} + \epsilon \approx 3.943$, and $5$ for diversity-aware $k$-median, diversity-aware $k$-means and diversity-aware $k$-supplier, respectively. Assuming Gap-ETH, the approximation ratios are tight for the diversity-aware $k$-median and diversity-aware $k$-means problems. Our results imply the same approximation factors for their respective fair variants with disjoint groups -- fair $k$-median, fair $k$-means, and fair $k$-supplier -- with lower bound requirements.

==> tikz/tikz-defs.tex <==
\tikzstyle{exedge}  = [draw = black, ultra thick, text=black]
\tikzstyle{exedget} = [draw = yafcolor5!20, thick, text=black!20]
\tikzstyle{exedgedir} = [draw = yafcolor5!20, thick, text=black!20, latex-latexnew, arrowhead=5mm]

\tikzstyle{exnode}  = [thick, draw = black, fill=yafcolor2!05, font = \large,  circle, inner sep = 1pt, text=black, minimum width=14pt]
\tikzstyle{exnodet} = [thick, draw = yafcolor4!20, fill=yafcolor2!02, font = \large,  circle, inner sep = 1pt, text=black!20, minimum width=14pt]
\tikzstyle{exlabel} = [circle, inner sep = 1pt,  font = \large, text = black, auto]
\tikzstyle{exsource}  = [thick, draw = red, fill=yafcolor2!05, font =\large, inner sep = 1pt, text=black, minimum width=14pt, minimum height=14pt]
\tikzstyle{exsquare}  = [thick, draw = yafcolor4!20, fill=yafcolor2!05, font =\large, inner sep = 1pt, text=black, minimum width=14pt, minimum height=14pt]
\tikzstyle{exdiamond}  = [thick, draw = yafcolor4!20, fill=yafcolor2!05, font =\large, inner sep = 1pt, diamond, text=black, minimum width=18pt, minimum height=18pt]

\tikzstyle{label}  = [fill=white, minimum width=0pt, inner sep = 0pt]


\tikzstyle{node1}  = [thick, draw = yafcolor1!100, fill=yafcolor1!05, circle, inner sep = 2.8pt]
\tikzstyle{node2}  = [thick, draw = yafcolor2!100, fill=yafcolor2!05, circle, inner sep = 2.8pt]
\tikzstyle{node3}  = [thick, draw = yafcolor3!100, fill=yafcolor3!05, circle, inner sep = 2.8pt]
\tikzstyle{node4}  = [thick, draw = yafcolor4!100, fill=yafcolor4!05, circle, inner sep = 2.8pt]
\tikzstyle{node5}  = [thick, draw = yafcolor5!100, fill=yafcolor5!05, circle, inner sep = 2.8pt]
\tikzstyle{node7}  = [thick, draw = yafcolor7!100, fill=yafcolor7!05, circle, inner sep = 2.8pt]
\tikzstyle{node8}  = [thick, draw = yafcolor8!100, fill=yafcolor8!05, circle, inner sep = 2.8pt]


\tikzstyle{node}  = [thick, draw = black!100, fill=yafcolor2!05, font = \large,  circle, inner sep = 1pt, text=black, minimum width=14pt]
\tikzstyle{mnode}  = [thick, draw = black!100, fill=yafcolor2!05, font = \large,  circle, inner sep = 1pt, text=black, minimum width=10pt]

\tikzstyle{fcircle}  = [thick, draw = black!100, font = \large,
circle, inner sep = 1pt, text=black, minimum width=4cm]
\tikzstyle{dcircle}  = [loosely dotted, ultra thick, draw = red, font = \large,
circle, inner sep = 1pt, text=black, minimum width=4cm]

\tikzstyle{point1}  = [draw = yafcolor1!100, fill=black, circle, inner sep=2pt]
\tikzstyle{point2}  = [draw = red, fill=red, circle, inner sep=2pt]

